A Case for Lifetime Reliability-Aware Neuromorphic Computing

Neuromorphic computing with non-volatile memory (NVM) can significantly improve performance and lower energy consumption of machine learning tasks implemented using spike-based computations and bio-inspired learning algorithms. High voltages required to operate certain NVMs such as phase-change memory (PCM) can accelerate aging in a neuron's CMOS circuit, thereby reducing the lifetime of neuromorphic hardware. In this work, we evaluate the long-term, i.e., lifetime reliability impact of executing state-of-the-art machine learning tasks on a neuromorphic hardware, considering failure models such as negative bias temperature instability (NBTI) and time-dependent dielectric breakdown (TDDB). Based on such formulation, we show the reliability-performance trade-off obtained due to periodic relaxation of neuromorphic circuits, i.e., a stop-and-go style of neuromorphic computing.

==> sections/background.tex <==
{SNN} is a network of neurons interconnected via synapses. Neurons are implemented using the Integrate-and-Fire (I\&F) model~\cite{indiveri2003low}. In this model, the membrane voltage (called action potential) of a post-synaptic neuron increases due to the current injected at its input from its pre-synaptic neurons after propagating (modulation) through the corresponding synaptic weight between the pre- and post-synaptic neuron. 
A neuron fires a spike when its membrane voltage exceeds a threshold and subsequently the membrane voltage is reset. The moment of threshold crossing defines the \textit{firing time} of the post-synaptic neuron. In Figure~\ref{fig:snn_ex}, we illustrate a simple SNN with two pre-synaptic neurons \ineq{n_i} and \ineq{n_j} connected to a post-synaptic neuron \ineq{n_k} via the synaptic weights \ineq{w_{i,k}} and \ineq{w_{j,k}}, respectively. A key characteristic of spiking neurons is their \textit{refractory period}. This refers to a brief rest period after a spike is fired, when the neuron is unable to fire again. Schematically, this is shown in the figure in the box labeled \ineq{\varphi}. Figure \ref{fig:neuron} shows the very large scale integration (VLSI) circuit implementation of an I\&F neuron~\cite{indiveri2003low}. As can be seen from this figure, a neuron consists of several CMOS devices, which age over time when exposed to an overdrive voltage.\footnote{Overdrive voltage is defined as the voltage between the gate and source terminals ($V_{GS}$) of a CMOS device in excess of its threshold voltage ($V_\text{th}$), where $V_\text{th}$ is the minimum voltage required to turn the device on.}

\begin{figure}[htbp]%
	\centering
	\subfloat[][An example SNN. \label{fig:snn_ex}]{
		\includegraphics[width=0.3\columnwidth]{images/snn_example.pdf}
	}
	\quad
	\subfloat[][VLSI implementation of a neuron~\cite{indiveri2003low}. \label{fig:neuron}]{
		\includegraphics[width=0.6\columnwidth]{images/neuron.pdf}
	}
	\caption{(a) A simple SNN with two pre-synaptic neurons connected to a post-synaptic neuron  and (b) VLSI implementation of an I\&F neuron~\cite{indiveri2003low}.}
	\label{fig:snn_neuron}
\end{figure}

Figure~\ref{fig:crossbar} illustrates a representative crossbar architecture that maps and executes SNNs. A crossbar is a 3D organization of rows (top electrodes or TEs) and columns (bottom electrodes or BEs), with NVM cells connected at their intersection, i.e., at the crosspoint of a row and a column. A pre-synaptic neuron is mapped on a TE and a post-synaptic neuron on a BE. The synaptic weight between a pre- and a post-synaptic neuron is programmed as conductance of the corresponding NVM cell at the crosspoint. The pre-synaptic neuron's voltage (applied along the TE) is multiplied by the conductance to generate current (following Ohm's Law). This current propagates to the post-synaptic neuron to raise its action potential. Current summation occurs on the BEs following Kirchoff's Current Law, when integrating excitation from other pre-synaptic neurons.


\begin{figure}[htbp]%
	\centering
	\vspace{-10pt}
	\subfloat[][A crossbar with top and bottom electrodes integrating NVM cells. \label{fig:crossbar}]{
		\includegraphics[width=0.5\columnwidth]{images/crossbar.pdf}
	}
	\quad
	\subfloat[][Mapping of the SNN example in Figure \ref{fig:snn_ex} to the crossbar. \label{fig:mapping}]{
		\includegraphics[width=0.4\columnwidth]{images/crossbar2.pdf}
	}
	\caption{(a) A crossbar based architecture to map and exeute SNN  and (b) Mapping of the SNN example in Figure~\ref{fig:snn_ex} to the crossbar.}
	\label{fig:crossbar_mapping}
	\vspace{-10pt}
\end{figure}

Figure~\ref{fig:mapping} shows a 2D view of the example SNN of Figure~\ref{fig:snn_ex} mapped on to the crossbar. The synaptic weights \ineq{w_{i,k}} and \ineq{w_{j,k}} are programmed as conductance of two NVM cells. Without loss of generality, we use input ports 1 and 2 to map the pre-synaptic neurons \ineq{n_i} and \ineq{n_j}, respectively. The output port 4 is used to map the post-synaptic neuron \ineq{n_o}.

Modern neuromorphic hardware platforms integrate many crossbars to map large SNNs. The crossbars are typically interconnected using a shared bus or a Network-on-Chip (NoC).
Using this relevant background, we now discuss aging-related reliability issues in crossbars of neuromorphic hardware.


